Language-aware Indexing for Conjunctive Path Queries

Conjunctive path queries (CPQ) are one of the most frequently used queries for complex graph analysis. However, current graph indexes are not tailored to fully support the power of query languages to express CPQs. Consequently, current methods do not take advantage of significant pruning opportunities during \cpq{} evaluation, resulting in poor query processing performance. We propose the CPQ-aware path index CPQx, the first path index tailored to the expressivity of CPQ. CPQx is built on the partition of the set of source-target vertex pairs of paths in a graph based on the structural notion of path-bisimulation. Path-bisimulation is an equivalence relation on paths such that each partition block induced by the relation consists of paths in the graph indistinguishable with respect to CPQs. This language-aware partitioning of the graph can significantly reduce the cost of query evaluation. We present methods to support the full index life cycle: index construction, maintenance, and query processing with our index. We also develop interest-aware CPQx to reduce index size and index construction overhead while accelerating query evaluation for queries of interest. We demonstrate through extensive experiments on 14 real graphs that our methods accelerate query processing by up to multiple orders of magnitude over the state-of-the-art methods, with smaller index sizes. Our complete C++ codebase is available as open source for further research.

==> 06.experiments.tex <==
\section{Experimental Study}
\label{sec:experiment}
We next present the results of an experimental evaluation of our methods.
We designed the experiments to clarify the questions:
(1) Does \CPQ-aware indexing
accelerate query processing?  (Section \ref{ssec:exp_efficiency});
(2) Are \CPQ-aware indexes compact? (Section \ref{ssec:exp_scalability}); and,
(3) Are \CPQ-aware indexes maintainable? (Section \ref{ssec:exp_update}).
%; and,
%(4) {\em Are CPQ-aware indexes well-behaved as $k$ grows?} (Section \ref{ssec:exp_analysis}).
{\it An extended report in our Github repository shows more experimental results (e.g., the impact of $k$ and scalability on synthetic datasets).}
%(4) {\em Are structural indexes well-behaved as $k$ grows?} (Section \ref{ssec:exp_analysis}).
%(4) {\em Are structural indexes well-behaved as $k$ and $|\elabels|$ grow?} (Section \ref{ssec:exp_analysis}).


\input{querytemplates_tikz.tex}
\begin{figure*}[ttt]
\centering
\begin{minipage}[t]{1.0\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/experiment/overview_query_legends.pdf}
    \end{minipage}
    \\
\begin{minipage}[t]{1.0\linewidth}
    \centering
	\includegraphics[width=1.0\linewidth]{figures/experiment/overview_query_color.pdf}
	\vspace{-9 mm}
	\caption{Average query time for 12 query templates. We terminated queries if the queries did not finish within two hours. 
    Note that \cpqindex{} and Path are not reported for WikiTalk, YAGO, CitPatents, Wikidata, and Freebase due to out of memory.}
    \vspace{-4mm}
	\label{fig:querytime}
	\end{minipage}
\end{figure*}

\begin{table}[]
    \centering
    \caption{Dataset overview: $|\edges|$ and $|\elabels|$ include inverse edges and labels, respectively.}
    \vspace{-3mm}
    \label{tab:dataset}
    {\footnotesize
    \begin{tabular}{|c|r|r|r|c|}\hline
         Dataset  &\multicolumn{1}{|c|}{$|\vertices|$} & \multicolumn{1}{|c|}{$|\edges|$} & \multicolumn{1}{|c|}{$|\elabels|$}&Real label?\\ \Hline
         {\bf Robots} & 1{,}484 & 5{,}920 & 8&\checkmark\\
         {\bf ego-Facebook} & 4{,}039 & 176{,}468 & 16& \\
         {\bf Advogato} & 5{,}417 & 102{,}654 & 8&\checkmark \\         
         {\bf Youtube}& 15{,}088 & 21{,}452{,}214 & 10&\checkmark \\    
         {\bf StringHS} & 16{,}956 & 2{,}483{,}530 & 14&\checkmark\\  
         {\bf StringFC} & 15{,}515 & 4{,}089{,}600 & 14&\checkmark \\         
         {\bf BioGrid} & 64{,}332 & 1{,}724{,}554 & 14&\checkmark\\              
         {\bf Epnions} & 131{,}828 & 1{,}681{,}598 & 16& \\
         {\bf WebGoogle}& 875{,}713 & 10{,}210{,}074 & 16&  \\     
         {\bf WikiTalk}& 2{,}394{,}385 & 10{,}042{,}820& 16&  \\      
         {\bf YAGO}& 4{,}295{,}825 & 24{,}861{,}400 & 74&\checkmark\\
         {\bf CitPatents}& 3{,}774{,}768 & 33{,}037{,}896 & 16& \\ 
         {\bf Wikidata}& 9{,}292{,}714 & 110{,}851{,}582 & 1054&\checkmark \\
         {\bf Freebase}& 14{,}420{,}276 & 213{,}225{,}620 & 1556 &\checkmark \\\hline 
        %  {\bf g-Mark-1m} & 1{,}006{,}802 & 15{,}925{,}506 & 12& \\
        %  {\bf g-Mark-5m} & 5{,}005{,}992 & 84{,}994{,}500 & 12& \\
        %  {\bf g-Mark-10m} & 10{,}005{,}721 & 183{,}748{,}319 & 12& \\
        %  {\bf g-Mark-15m} & 15{,}003{,}647 & 255{,}538{,}724 & 12& \\
        %  {\bf g-Mark-20m} & 20{,}004{,}856 & 393{,}797{,}046 & 12& \\\hline
    \end{tabular}
    }
        \vspace{-3mm}
\end{table}

Experiments were performed on a Linux server with 512GB of memory and an Intel(R) Xeon(R) CPU E5-2699v3 processor. All algorithms are single-threaded.
%Experiments were performed on a Linux server with 512GB of memory and an Intel(R) Xeon(R) CPU E5-2699v3@2.30GHz processor. All algorithms are single-threaded.



\smallskip
\noindent {\bf Datasets.} 
Table \ref{tab:dataset} provides an overview of the datasets used in our study consisting of nine datasets with real labels and five datasets without edge labels.
The graphs range over several different scenarios, such as social networks, biological networks, and knowledge graphs.
These datasets are provided by the authors~\cite{Valstar2017,peng2020answering} except for ego-Facebook, webGoogle, WebTalk, CitPatents, and Wikidata. 
In Wikidata, we extract vertices that represent URI from original Wikidata~\cite{Wikidata}.
%\footnote{\url{https://www.wikidata.org/}}
ego-Facebook, WebGoogle, WebTalk, and CitPatents are available at SNAP~\cite{snap}.
%\footnote{http://snap.stanford.edu/}.
%, and five synthetic datasets generated by the state-of-the-art gMark graph generator \cite{bagan2016gmark}.
%The graphs range over several different scenarios, such as hyperlinks, social networks, and knowledge graphs. 
Since these four graphs have no edge labels, we assign edge labels that are exponentially distributed with $\lambda = 0.5$ which follows the distribution of edge labels on YAGO.
%As StringHS and StringFC often have similar result trends, we omit the results of StringHS at some points due to space constraints.
Note that the graphs are of the same size and complexity as those used in recent studies \cite{han2019efficient,Valstar2017,peng2020answering,sun2020rapidmatch}.
%of path queries and subgraph matching \cite{han2019efficient,Valstar2017,peng2020answering,sun2020rapidmatch}.


% The synthetic datasets model citation networks with three types of vertices, {\edgefont researcher}, {\edgefont venue}, and {\edgefont city}, and six edge labels, {\edgefont cites} from/to researchers, {\edgefont supervises} from/to researchers, {\edgefont livesIn} from researcher to city, {\edgefont workisIn} from researcher to city, {\edgefont publishesIn} from researcher to venue, and {\edgefont heldIn} from venue to city.
% We use the synthetic datasets for evaluating scalability, varying the number of vertices and edges from roughly 1 and 8 million ({\bf g-Mark-1m}) to 20 and 200 million ({\bf g-Mark-20m}), resp.

\smallskip
\noindent {\bf Queries.} 
We used twelve \CPQ{} templates as described in Figure~\ref{fig:querytemplates}.
These query structures correspond to practical structures appearing, e.g., in the Wikidata query logs \cite{bonifati2020analytical, BonifatiMT19}.
We use as abbreviations C, T, S, and St for Chain, Triangle, Square, and Star, respectively. 
We especially chose these templates to (1) better understand the interaction of all basic constructs of the language and (2) exemplify query structures occurring frequently in practice such as chains (e.g., C4), stars (St), cycles (e.g., Ti), and flowers (e.g., ST).


%The design rationale of these templates is to isolate and study the different basic operations of the language and their combined use.

%We categorize these templates into those using $\cmp$  ({\sf C2} and {\sf C4}), those using both $\cmp$ and $\cap$ ({\sf T}, {\sf S}, {\sf TT}, {\sf TC}, {\sf SC}, and {\sf ST}), and those using $\cmp$, $\cap$, and $\identity$ ({\sf C2i}, {\sf Ti}, {\sf Si}, and {\sf St}).
% Path indexes process paths of length at most $k$ without physical joins (i.e., $\cmp$), so we 
% %can further refine our classification 
% categorize these templates into six categories when $k>1$:
% (a) queries without joins and with conjunction ({\sf T}, {\sf S}, {\sf TT}, and {\sf St}), 
% (b) queries with joins and conjunction  ({\sf TC}, {\sf SC}, and {\sf ST}),
% (c) queries with join and without conjunction ({\sf C4})
% (d) queries with join and identity ({\sf Ti} and {\sf Si})
% (e) queries only with lookup ({\sf C2}), and
% (f) queries only with lookup and identity ({\sf C2i}).

%Our index has advantage for queries with conjunction and without join.
%because they include only conjunction when we set $k$ is larger than or equal to two.
%On the other hand, the path index has advantage for queries with join and without conjunction.
%four queries, {\sf C2}, {\sf C4}, {\sf Ti}, and {\sf Si} because they do not include conjunction. 

For each template and dataset, we generate ten queries with random labels.
%, with a mix of queries having empty and non-empty result sets. 
%We evaluate each query three times and record the middle response time. 
We only use queries in which all (sub-)paths of length two are non-empty, but the answers of some queries may be empty.
To evaluate the difference between query times of non-empty and empty queries, queries on Yago, Wikidata, and Freebase have 50$\%$ non-empty and 50$\%$ empty queries except for C2. Queries for other datasets consist of mostly non-empty queries though we randomly set labels.
We report for each query template the average response time over all ten queries.
Note that the answers of some queries may be empty, but intermediate results are non-empty.



\noop{
\begin{table}[]
    \centering
    \caption{Dataset overview}
    \label{tab:dataset}
    {\small
    \begin{tabular}{|c|r|r|r|c|}\hline
         Dataset  &\multicolumn{1}{|c|}{$|\vertices|$} & \multicolumn{1}{|c|}{$|\edges|$} & \multicolumn{1}{|c|}{$|\elabels|$}&Real label?\\ \Hline
         {\bf Robots}\footnotemark[3] & 1{,}484 & 2{,}960 & 4&\checkmark\\
         {\bf Advogato}\footnotemark[4] & 5{,}417 & 51{,}327 & 4&\checkmark \\
         {\bf BioGrid}\footnotemark[5] & 64{,}332 & 862{,}277 & 7&\checkmark\\       
         {\bf StringHS}\footnotemark[6] & 16{,}956 & 1{,}241{,}765 & 7&\checkmark\\  
         {\bf StringFC}\footnotemark[6] & 15{,}515 & 2{,}044{,}800 & 7&\checkmark \\
         {\bf WikiTalk}\footnotemark[9]& 2{,}394{,}385 & 5{,}021{,}410& 8&  \\       
         {\bf WebGoogle}\footnotemark[9]& 875{,}713 & 5{,}105{,}037 & 8&  \\
         {\bf Youtube}\footnotemark[7] & 15{,}088 & 10{,}726{,}107 & 5&\checkmark \\ 
         {\bf YAGO}\footnotemark[8]& 4{,}295{,}825 & 12{,}430{,}700 & 37&\checkmark\\
         {\bf CitPatents}\footnotemark[9]& 3{,}774{,}768 & 16{,}518{,}948 & 8& \\ 
         {\bf Freebase}\footnotemark[10]& 14{,}420{,}276 & 106{,}612{,}810 & 778 &\checkmark \\ 
         {\bf g-Mark-1m} & 1{,}006{,}802 & 7{,}962{,}753 & 6& \\
         {\bf g-Mark-5m} & 5{,}005{,}992 & 42{,}497{,}250 & 6& \\
         {\bf g-Mark-10m} & 10{,}005{,}721 & 91{,}874{,}159 & 6& \\
         {\bf g-Mark-15m} & 15{,}003{,}647 & 127{,}769{,}362 & 6& \\
         {\bf g-Mark-20m} & 20{,}004{,}856 & 196{,}898{,}523 & 6& \\\hline
    \end{tabular}
    }
\end{table}
\footnotetext[3]{http://tinyurl.com/gnexfoy}
\footnotetext[4]{http://konect.uni-koblenz.de/}
\footnotetext[5]{http://thebiogrid.org}
\footnotetext[6]{http://string-db.org}
\footnotetext[7]{http://socialcomputing.asu.edu./datasets/Youtube}
\footnotetext[8]{https://datahub.io/collections/yago}
\footnotetext[9]{http://snap.stanford.edu/}
\footnotetext[10]{https://developers.google.com/freebase}
}


\smallskip

\noindent {\bf Methods.} We compare the following methods: 
    {\bf \cpqindex}, our \CPQ-aware index of Section \ref{sec:index};
    {\bf \iacpqindex}, our interest-aware \cpqindex{} of Section \ref{sec:workload};
    {\bf Path}, the state-of-the-art language-unaware path index proposed in \cite{fletcher2016efficient}; 
    {\bf iaPath}, {\bf Path} where only label sequences included in the given interest are indexed; 
    {\bf TurboHom++}, the state-of-the-art algorithm for homomorphic subgraph matching \cite{kim2015taming}\footnote{The binary code of TurboHom++ was provided by the authors \cite{kim2015taming}.}; 
    {\bf Tentris}, the state-of-the-art RDF engine~\cite{bigerl2020tentris}\footnote{\url{https://github.com/dice-group/tentris}}; and,
    {\bf BFS}, index-free breadth-first-search query evaluation \cite{Bonifati2018}.
    We implemented all methods (see our open source codebase) except for TurboHom++ and Tentris.
    %for which we used the authors' binary code \cite{kim2015taming}. 
    To be fair, we used the same query plans for all methods, except for TurboHom++ and Tentris which perform their own planning. 
    %We note that the implementation of TurboHom++ just counts the number of answers, while others output all answers, so our method is more expensive in this sense.
    % urboHom++ searches for subgraphs instead of paths, so its search space is larger than that of \cpq. To fairly compare our methods with {\bf TurboHom++}, we evaluate the query time for finding the first answer (see Fig. \ref{fig:negaposi}). 
    
    
    %We also tested an , but its performance is significantly lower than TurboHom++ and Tentris. 
    A {\bf relational database approach} is essentially the same as Path with $k=1$, which has lower performance than with $k=2$.
    {\bf RDF3X} and {\bf Virtuoso} were shown to be outperformed by TurboHom++~\cite{kim2015taming} and Tentris~\cite{bigerl2020tentris}.
    %RDF systems with structural index such as gStore \cite{zou2011gstore} are not publicly available.
    Thus, we exclude Virtuoso, RDF3X, and the relational graph approach in our experiments.
    %do not show these results of virtuoro and relational graph approach due to space limitation.



%We varied path length $k$ from one to four, with a default value of two.
We set path length $k$ as two.
For the interest-aware indexes, we specify all label sequences in the set of queries as the interests. We divide label sequences of length larger than two into prefix label sequences of length two and the rest.
% On synthetic datasets, we specify five label sequences as interests; {\edgefont cites}-{\edgefont cites}, {\edgefont cites}-{\edgefont supervises}, {\edgefont publishesIn}-{\edgefont heldIn}, {\edgefont worksIn}-{\edgefont heldIn}$^{-1}$, and {\edgefont livesIn}-{\edgefont worksIn}$^{-1}$.



% \smallskip

% \noindent
% {\bf Index implementation.} 
% In this study we use simple in-memory data structures;
% the study of alternative physical index representations is an interesting topic beyond the scope of this paper.
% Identifiers of vertices and labels are 32-bit integers.
% Indexes are implemented as standard C++ vectors. For further details, please see our open-source codebase. 




%The optimization of physical index representation is an interesting topic beyond the scope of this paper.

% \subsection{An overview of Performance}

% We show an overview of performance in terms of query time, indexing time, and index size.
% Consequently, our proposal accelerates query processing up to four orders of magnitude than the path index. Furthermore, our index achieves smaller size of index than the path index.







%          {\bf g-Mark-1m}  & 0.4 & 79.6 & 0.8 & 166.7\\
%          {\bf g-Mark-5m}  & 2.6 & 547.4 & 5.0 & 1005.7\\
%          {\bf g-Mark-10m} & 5.6 & 1367.7 & 12.0 & 2478.0 \\
%          {\bf g-Mark-15m} & 7.8 & 5989.4  & - & - \\
%          {\bf g-Mark-20m} & 13.0 & 3380.5 & 26.0 & 7491.4 \\\hline




\begin{figure*}[ttt]
\begin{tabular}{cc}
  \begin{minipage}{.39\textwidth}
  %\vspace{-13mm}
  \centering
\tblcaption{The numbers of class identifiers on \cpqindex{} and \iacpqindex{} and the number of s-t pairs on iaPath, for evaluating S queries. 
%We note that Path and IA-Path indexes search for the same number of paths on queries.
}
%\caption{The difference between the numbers of class identifiers and paths.}
\label{tab:numhistory}
{\footnotesize
\begin{tabular}{|c|r|r|r|}\hline
      \multicolumn{1}{|c|}{Dataset}&\multicolumn{1}{|c|}{\cpqindex} &\multicolumn{1}{|c}{\iacpqindex}&\multicolumn{1}{|c|}{iaPath}\\ \Hline
     {\bf Robots} & 0.4K & 0.13K  &  2.4K \\
     {\bf ego-Facebook} &22K & 19K &  23K \\
     {\bf Youtube} & 18M & 2.0M &  21M\\
     {\bf Epinions} &715K & 222K  &  1.8M \\
     {\bf Advogato} & 38.0K & 6.4K &  93.6K \\
     {\bf BioGrid} & 275K & 71.2K  &  499K \\         
     {\bf StringHS} & 49.7K & 11.2K&  750K \\        
     {\bf StringFC} & 33.3K & 3.7K&  388K\\
     {\bf Yago} & - & 75 &  967K\\     
     {\bf WikiTalk} &- & 915K &  19M\\  
     {\bf WebGoogle} & - & 287K &  760K\\  
     {\bf CitPatents} & - & 36K &   1.1M \\
     {\bf Wikidata} & - & 3 & 286M\\ 
     {\bf Freebase} & - & 8.6 &   79K \\
     \hline
\end{tabular}
}
  \end{minipage}
  \quad
  \begin{minipage}{.55\textwidth}
  \begin{minipage}[t]{1.0\linewidth}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/experiment/negaposi_legends_full.pdf}
\end{minipage}
\\
\begin{minipage}[t]{1.0\linewidth}
     \centering
     \vspace{-3mm}
  \subfloat[Yago]{\epsfig{file=./figures/experiment/negaposi_yago_full.pdf,width=1.0\linewidth}
  }\\
       \vspace{-3mm}
  \subfloat[Wikidata]{\epsfig{file=./figures/experiment/negaposi_wikidata_full.pdf,width=1.0\linewidth}
  }\\
       \vspace{-3mm}
\subfloat[Freebase]{\epsfig{file=./figures/experiment/negaposi_freebase_full.pdf,width=1.0\linewidth}
  }
\end{minipage}
\vspace{-2mm}
  \caption{Average query time of empty and non-empty queries, and for obtaining the first result of non-empty queries}
 \label{fig:negaposi}
  \end{minipage}
\end{tabular}
\vspace{-2mm}
\end{figure*}

\subsection{Does CPQ-aware indexing accelerate query processing? }
\label{ssec:exp_efficiency}



In summary, we can answer ``yes'' for this question.
Figure \ref{fig:querytime} shows the average query time of each method for each of the twelve query templates on nine datasets.
We do not show results on other five datasets due to page limitation.

\CPQ-aware indexes accelerate {\sc Conjunction} as mentioned at Section \ref{ssec:query}, so query times of T, S, TT, and St with \cpqindex{} and \iacpqindex{} are significantly smaller than those with all methods.
%, up to thousands times faster on queries with {\sc Conjunction} and without {\sc Join}.
For TC, SC, and ST, either \iacpqindex{} or Path are the fastest on many datasets.
When {\sc Conjunction} is heavy, \iacpqindex{} is advantageous. 
For queries with {\sc Join} and without {\sc Conjunction} such as C2, C4, Ti, and Si, since \CPQ-aware indexes take two accesses to both $I_{l2c}$ and $I_{c2p}$, they have higher costs than Path, but the difference between them is small.
%So, Path is better than Structual on simple navigation queries such as C2 and C4.
Query time of C2i is smaller than that of C2 in both \iacpqindex{} and Path.
This is because the size of answers decreases, and thus a cost for inserting s-t pairs to the answer sets reduces.
Efficient {\sc Identity} works well on some datasets such as Robots, YAGO, and Freebase while the efficiency highly depends on specified labels.
For Ti and Si, TurboHom++ and Tentris perform well on some datasets because it joins only s-t pairs that satisfy cycle but other methods check whether s-t pairs are cycle or not after join. Tentris additionally performs well for St query on some dataset due to its query optimization.
Compared with TurboHom++ and Tentris, our methods have significant improvement for many query templates such as T, S, TT, St, C2, and C2i. In particular, TurboHom++ and Tentris do no finish some queries within two hours in experiments; whereas \iacpqindex{} and Path finish all queries within two hours.

Comparing \cpqindex{} with \iacpqindex, \iacpqindex{} is more efficient because the numbers of class identifiers is smaller.
In particular, for C2i, \iacpqindex{} is much faster than \cpqindex{} as it reduces the number of {\sc LookUp}. 
Here, we note that iaPath does not become faster than Path because both of the indexes have the same number of s-t pairs regarding to label sequences.

% From these results, we can see that the structural index achieves efficient query processing for conjunctive path queries.
% Furthermore, when we have specific interests, the interest-aware structural index accelerates evaluation of conjunctive path queries more.

%The structural index achieves faster query processing for conjunction operation.
%This is because our query processing algorithm compares class identifiers instead of paths.
%We here show the numbers of class identifiers and paths for Square queries.






% \begin{table*}[ttt]
%     \centering
%     \caption{Index size (IS), index time (IT), and memory usage for constructing indexes (IM), where ``-'' indicates out of memory.}
%     \vspace{-3mm}
%     \label{tab:index}
%     {\small
%     \begin{tabular}{|c|r|r|r|r|r|r|r|r|r|r|r|r|}\hline
%          \multirow{2}{*}{Dataset}& \multicolumn{3}{|c|}{\cpqindex}&\multicolumn{3}{|c|}{\iacpqindex}&\multicolumn{3}{|c|}{Path}&\multicolumn{3}{|c|}{iaPath}  \\
%           &\multicolumn{1}{c}{IS [B]}&\multicolumn{1}{c}{IT [s]}&\multicolumn{1}{c|}{IM [B]}&\multicolumn{1}{c}{IS [B]}&\multicolumn{1}{c}{IT [s]}&\multicolumn{1}{c|}{IM [B]}&\multicolumn{1}{|c}{IS [B]}&\multicolumn{1}{c}{IT [s]}&\multicolumn{1}{c|}{IM [B]}&\multicolumn{1}{|c}{IS [B]}&\multicolumn{1}{c}{IT [s]}&\multicolumn{1}{c|}{IM [B]}\\ \Hline
%          {\bf Robots}  & 1.78M& 0.26 & 84.0M & 0.46M & 0.056& 19.4M & 2.0M & 0.085& 35.0M & 0.52M & 0.043& 19.9M \\
%          {\bf ego-Facebook}  & 97.4M& 18.3 & 2.1G  & 15.4M  & 2.0 & 322.2M & 116.9M &6.0 & 974.3M & 20.9M & 131.5 & 324.1M \\
%          {\bf Youtube} & 27.6G& 57{,}653& 389.6G & 2.3G & 8{,}116& 103.3G & 34.0G & 28{,}870& 195.5G & 8.7G & 7{,}283 & 107.2G\\  
%          {\bf Advogato} & 56.7M& 11.9& 1.8G & 20.5M & 8.53& 752M & 74.4M  &3.5& 808M  & 29.0M & 2.3 & 754M\\
%          {\bf StringHS} & 1.4G& 521.4 & 71.0G & 1.3G & 335.9& 46.0G & 6.0G  & 260.4& 42.3G  & 2.8G &237.3 & 45.3G\\
%          {\bf StringFC} & 1.0G& 852.7& 60.4G& 0.97G & 664.7& 37.7G & 5.1G & 596.0& 36.6G  & 2.3G & 579.8& 37.5G\\
%          {\bf BioGrid}  & 1.7G& 495.1& 44.9G & 0.40G & 86.6& 10.1G& 2.48G & 137.0& 19.6G  & 0.63G & 47.9 & 10.1G\\
%          {\bf Epinions}  & 3.5G& 849.6 & 84.7G & 1.0G  & 229.6 & 25.3G & 4.5G & 264.1 & 36.6G & 1.3G & 122.8 & 25.3G \\
%          {\bf WebGoogle}  & - & -& -& 4.7G & 724.5& 93.8G & -& - & -  & 5.2G & 444.7 & 94.1G\\
%          {\bf WikiTalk}  & - & -& -& 14.4G & 3{,}064& 286.2G& - & - & -  & 16.0G & 1{,}060& 278.6G\\
%          {\bf YAGO}  & - & -& -& 3.8G & 809.4&68.8G & -& - & -  & 3.9G & 589.7& 67.6G\\
%          {\bf CitPatents}  & - & -& -& 2.2G & 469.5& 45.5G & -& - & -  & 2.5G & 226.4& 46.5G\\
%          {\bf Wikidata}  & - & -& -& 1.44G & 267.5&29.4G & -& - & -  & 1.47G & 70.4& 33.0G\\
%          {\bf Freebase}  & - & -& -& 1.0G & 5{,}696& 48.8G & -& - & -  & 3.7G & 5{,}176& 53.1G\\\hline
%          %{\bf g-Mark-1m}  & - & -&-& 0.63G & 104.9 & 13.6G & -  &-&-& 0.64M & 55.7&13.9G\\
%          %{\bf g-Mark-5m} & - & - &-& 4.1G & 728.0& 64.2G  & - &-&-& 4.1G & 257.4&65.4G\\
%          %{\bf g-Mark-10m}  & - & - &-& 9.3G & 1{,}715& 	167.3G & - &-&-& 9.4G & 574.2 &171.3G\\
%          %{\bf g-Mark-15m} & -& -  &-& 13.8G & 2{,}741 & 201.9G  & -  &-&-& 13.9G & 862.5 &204.1G\\
%          %{\bf g-Mark-20m} & -& -&-& 20.3G& 4{,}251& 337.9G & -  &-&-& 20.6G & 1{,}590&346.0G\\\hline
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[ttt]
    \centering
    \caption{Index size (IS) and index construction time (IT), where ``-'' indicates out of memory.}
    %\vspace{-3mm}
    \label{tab:index}
    {\footnotesize
    \begin{tabular}{|c|r|r|r|r|r|r|r|r|}\hline
         \multirow{2}{*}{Dataset}& \multicolumn{2}{|c|}{\cpqindex}&\multicolumn{2}{|c|}{\iacpqindex}&\multicolumn{2}{|c|}{Path}&\multicolumn{2}{|c|}{iaPath}  \\
          &\multicolumn{1}{c}{IS [B]}&\multicolumn{1}{c|}{IT [s]}&\multicolumn{1}{c}{IS [B]}&\multicolumn{1}{c|}{IT [s]}&\multicolumn{1}{|c}{IS [B]}&\multicolumn{1}{c|}{IT [s]}&\multicolumn{1}{|c}{IS [B]}&\multicolumn{1}{c|}{IT [s]}\\ \Hline
         {\bf Robots}  & 1.78M& 0.26  & 0.46M & 0.056 & 2.0M & 0.085& 0.52M & 0.043 \\
         {\bf ego-Facebook}  & 97.4M& 18.3  & 15.4M  & 2.0  & 116.9M &6.0  & 20.9M & 131.5  \\
         {\bf Youtube} & 27.6G& 57{,}653 & 2.3G & 8{,}116 & 34.0G & 28{,}870 & 8.7G & 7{,}283 \\  
         {\bf Advogato} & 56.7M& 11.9& 20.5M & 8.53 & 74.4M  &3.5  & 29.0M & 2.3\\
         {\bf StringHS} & 1.4G& 521.4  & 1.3G & 335.9 & 6.0G  & 260.4  & 2.8G &237.3\\
         {\bf StringFC} & 1.0G& 852.7& 0.97G & 664.7 & 5.1G & 596.0  & 2.3G & 579.8\\
         {\bf BioGrid}  & 1.7G& 495.1& 0.40G & 86.6& 2.5G & 137.0& 0.63G & 47.9 \\
         {\bf Epinions}  & 3.5G& 849.6 &1.0G  & 229.6  & 4.5G & 264.1 & 1.3G & 122.8\\
         {\bf WebGoogle}  & - & -& 4.7G & 724.5& - & -  & 5.2G & 444.7\\
         {\bf WikiTalk}   & -& -& 14.4G & 3{,}064 & - & -  & 16.0G & 1{,}060\\
         {\bf YAGO}  & - & -&3.8G & 809.4& - & -  & 3.9G & 589.7\\
         {\bf CitPatents}  & - &  -& 2.2G & 469.5& - & -  & 2.5G & 226.4\\
         {\bf Wikidata}  & - & -& 1.44G & 267.5& - & -  & 1.47G & 70.4\\
         {\bf Freebase}  & - & -& 1.0G & 5{,}696& - & -  & 3.7G & 5{,}176\\\hline
         
         %{\bf g-Mark-1m}  & - & -&-& 0.63G & 104.9 & 13.6G & -  &-&-& 0.64M & 55.7&13.9G\\
         %{\bf g-Mark-5m} & - & - &-& 4.1G & 728.0& 64.2G  & - &-&-& 4.1G & 257.4&65.4G\\
         %{\bf g-Mark-10m}  & - & - &-& 9.3G & 1{,}715& 	167.3G & - &-&-& 9.4G & 574.2 &171.3G\\
         %{\bf g-Mark-15m} & -& -  &-& 13.8G & 2{,}741 & 201.9G  & -  &-&-& 13.9G & 862.5 &204.1G\\
         %{\bf g-Mark-20m} & -& -&-& 20.3G& 4{,}251& 337.9G & -  &-&-& 20.6G & 1{,}590&346.0G\\\hline
    \end{tabular}
    }
\end{table*}



%\smallskip
\noindent
{\bf Pruning power.} We show the reason why our \CPQ-aware indexes accelerate query processing more than the-state-of-the-art language-unaware path indexes. 
Recall that our query processing algorithm accelerates queries with {\sc Conjunction} by comparing class identifiers instead of s-t pairs. 
Table \ref{tab:numhistory} shows the average numbers of class identifiers in \cpqindex{} and \iacpqindex{} and the average number of s-t pairs in iaPath, which are involved on evaluating S queries. 
The smaller numbers indicate higher pruning power. 

The numbers of class identifiers that are involved during the query evaluation in \cpqindex{} and \iacpqindex{} are much smaller than the number of s-t pairs in iaPath.
This result shows that partitioning s-t pairs based on $k$-path-bisimulation is effective for evaluating \CPQ. 


%\smallskip
\noindent
{\bf Impact of empty and non-empty queries.} We evaluate the impact of empty and non-empty results on query time.
The purposes here are (1) to gain further insight into the performance of our methods and (2) to compare the search strategy of our algorithm with that of TurboHom++ and Tentris. 
%TurboHom++ searches for answers by a depth-first manner, which is fast to find the first result, while our query algorithm only reports answers after the last logical operator.
Figure \ref{fig:negaposi} shows the query time on empty and non-empty queries on Yago, Wikidata, and Freebase of \iacpqindex{}, TurboHom++, and Tentris. 
%In TurboHom++ all query nodes are given as output, whereas \cpq's have binary output. 
TurboHom++ outputs subgraphs, whereas \CPQ s have binary output (i.e., s-t pairs). 
For a closer comparison, we also evaluate the query time for finding the first answer (thereby offsetting the cost of enumerating all non-binary answers with TurboHom++), also shown in Figure \ref{fig:negaposi}.

%Additionally, we evaluate the query time for finding the first answer in non-empty queries, which can fairly evaluate the query time without the difference of query semantics.
From these results, we can see that \iacpqindex{} is much faster than TurboHom++ and Tentris for both empty and non-empty queries on most datasets and query templates.
%For finding the first answer in queries with {\sc Conjunction} (e.g., T and S), IA-Structural is faster than TurboHom++, so we can confirm that our methods are faster than TurboHom++ even though they have slightly different query semantics (i.e., binary or non-binary answers).
The query time on empty queries is generally smaller than that on non-empty queries because (1) empty queries do not have insert cost to the answers and (2) empty queries might terminate on the way of query evaluation due to empty intermediate results.
Some non-empty queries are faster than empty queries when the intermediate results on empty queries are large. 


%From these results, we confirm that the IA-structural achieves fast evaluation for both non-empty and empty queries.



% \begin{figure}[!t]
%   \centering
%   \subfloat[Yago]{\epsfig{file=./figures/negaposi_yago.pdf,width=1.0\linewidth}
%   }\\
% \subfloat[Freebase]{\epsfig{file=./figures/negaposi_freebase.pdf,width=1.0\linewidth} 
%   }
%   \caption{Query time of empty and non-empty queries}
%  \label{fig:negaposi}
% \end{figure}


% \begin{table}[!t]
% \centering
% \caption{The number of histories for Structural and IA-structural and the number of paths for Path on Square queries. We note that Path and IA-Path indexes search for the same number of paths on queries.}
% %\caption{The difference between the numbers of class identifiers and paths.}
% \label{tab:numhistory}
% {\small
% \begin{tabular}{|c|r|r|r|}\hline
%       \multicolumn{1}{|c|}{Dataset}&\multicolumn{1}{|c|}{Structural} &\multicolumn{1}{|c}{IA-Structural}&\multicolumn{1}{|c|}{Path}\\ \Hline
%      {\bf Robots} & 0.4K & 0.13K  &  2.4K \\
%      {\bf Advogato} & 38.0K & 6.4K &  93.6K \\
%      {\bf BioGrid} & 275K & 71.2K  &  499K \\         
%      {\bf StringHS} & 49.7K & 11.2K&  750K \\        
%      {\bf StringFC} & 33.3K & 3.7K&  388K\\
%      {\bf Youtube} & 18M & 2.0M &  21M\\
%      {\bf Yago} & - & 75 &  967K\\     
%      {\bf WikiTalk} &- & 915K &  19M\\  
%      {\bf WebGoogle} & - & 287K &  760K\\  
%      {\bf CitPatents} & - & 36K &   1.1M \\
%      {\bf Freebase} & - & 8.6 &   79K \\
%      \hline
% \end{tabular}
% }
% \end{table}

% \begin{figure}[ttt]
%   \centering
%   \includegraphics[width=0.8\linewidth]{figures/negaposi_yago.pdf}
%   \caption{Query time of empty and non-empty queries on Yago dataset}
%   \label{fig:negaposi}
% \end{figure}



% {\bf Scalability:} Figure \ref{fig:query_graphsize} shows the {\bf IA-Structural} average query time for varying graph size of synthetic datasets. Our method scalably evaluates $\cpq$s as graphs grow larger. 

% \begin{figure}[ttt]
% \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/graphsize_query_legends-crop.pdf}
% \end{minipage}
% \\
% \begin{minipage}[t]{0.8\linewidth}
%      \centering
%     \includegraphics[width=0.95\linewidth]{figures/graphsize_query_wastructural-crop.pdf}
% \end{minipage}
% \caption{IA-structural query performance as graph size grows}
% \label{fig:query_graphsize}
% \end{figure}


% \begin{table}[!t]
%     \centering
%     \caption{Update time on structural index}
%     \label{tab:maitenance_structural}
%     {\small
%     \begin{tabular}{|c|r|r|}\hline
%          \multirow{2}{*}{Dataset}  & \multicolumn{1}{|c|}{Edge} & \multicolumn{1}{|c|}{Edge} \\ 
%          & \multicolumn{1}{|c|}{deletion} & \multicolumn{1}{|c|}{insertion} \\\Hline
%          {\bf Robots}   & 0.0008 [s] & 0.0005 [s] \\
%          {\bf Advogato} & 0.005 [s] & 0.001 [s] \\
%          {\bf BioGrid}  & 0.6 [s] & 0.2 [s] \\         
%          {\bf StringHS} & 0.3 [s] & 0.1 [s]\\        
%          {\bf StringFC} & 0.2 [s] & 0.06 [s] \\
%          {\bf Youtube}  & 0.9 [s] & 0.3 [s]\\\hline
%     \end{tabular}
%     }
% \end{table}

\begin{table}
    \centering
    \caption{Update time on \iacpqindex}
    \label{tab:maitenance_wa_structural}
        %\vspace{-3mm}
    {\footnotesize
    \begin{tabular}{|c|r|r|r|r|}\hline
         \multirow{2}{*}{Dataset}  & \multicolumn{1}{|c|}{Edge} & \multicolumn{1}{|c|}{Edge} & \multicolumn{1}{|c|}{Interest} & \multicolumn{1}{|c|}{Interest} \\ 
         &\multicolumn{1}{|c|}{deletion}&\multicolumn{1}{|c|}{insertion}&\multicolumn{1}{|c|}{deletion}&\multicolumn{1}{|c|}{insertion}\\
         \Hline
         {\bf Robots}   & 0.2 [ms] & 0.1 [ms]& 0.2 [$\mu$s] & 0.01 [s] \\
         {\bf Advogato} & 0.004 [s] & 0.0004 [s]& 0.3 [$\mu$s] & 0.7 [s] \\
         {\bf BioGrid}  & 1.0 [s] & 0.005 [s]& 0.5 [$\mu$s] & 14.2 [s] \\         
         {\bf StringHS} & 0.2 [s] & 0.03 [s]& 0.5 [$\mu$s] & 15.4 [s]\\        
         {\bf StringFC} & 0.2 [s] & 0.04 [s]& 0.5 [$\mu$s] & 9.8 [s] \\
         {\bf Youtube}  & 1.2 [s] & 1.1 [s]& 0.5 [$\mu$s] & 255.5 [s]\\
         {\bf YAGO}  & 0.7 [s] & 0.04 [s]& 0.8 [$\mu$s] & 30.3 [s]\\
         {\bf Wikidata}  & 0.7 [s] & 0.4 [s]& 1.0 [$\mu$s] & 24.2 [s]\\         
         {\bf Freebase}  & 1.7 [s] & 0.2 [s]& 1.1 [$\mu$s] & 21.8 [s]\\
         \hline
    \end{tabular}
    }
%        \vspace{-5mm}
\end{table}

\begin{figure*}[ttt]
\begin{tabular}{ccc}
\begin{minipage}{.56\textwidth}
    \begin{minipage}[t]{1.0\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/experiment/k_query_legends.pdf}
\end{minipage}
\\
\begin{minipage}[t]{1.0\linewidth}
     \centering
      \includegraphics[width=0.9\linewidth]{figures/experiment/update_query_bisimulation.pdf}
      %\subfloat[Query Time for structural and IA-structural on graph update and IA-structural on interest update from left, respectively]{\epsfig{file=./figures/experiment/update_query_bisimulation.pdf,width=1.0\linewidth}}
\end{minipage}
    \vspace{-5mm}
    \caption{Impact of maintenance to query time on Robots}
    \label{fig:maintenance_querytime}
  \end{minipage}
  \begin{minipage}{.40\textwidth}
  \centering
      \vspace{-5mm}
\tblcaption{The increasing ratio of index size on update on Robots}
%\caption{The difference between the numbers of class identifiers and paths.}
\label{tab:maintenance_indexsize}
{\footnotesize
\begin{tabular}{|c|rrrrr|}\hline
    \multirow{2}{*}{Index}&\multicolumn{5}{|c|}{Ratio of updated edges}\\
        & 1 & 2 & 5 & 10 & 20 \\\hline
     \cpqindex &1.02& 1.04 & 1.11  &  1.35 & 1.63 \\
     \iacpqindex & 1.03 & 1.06 & 1.13 & 1.31 & 1.53 \\\hline\hline
     \multirow{2}{*}{Index}&\multicolumn{5}{|c|}{\# of updated interests}\\
     & 2 & 4 & 6 & 8 & 10 \\\hline
    \iacpqindex & 1.002 & 1.06  &  1.15 & 1.24 & 1.48 \\\hline
\end{tabular}
}
  \end{minipage}
\end{tabular}
\vspace{-5mm}
\end{figure*}



% Table \ref{tab:numhistory} shows the number of class identifiers in Structural and IA-Structural and the number of paths in Path.
% The numbers of class identifiers and paths have large gaps, in particular, StringHS and StringFC.
% This explains why Structural achieves much faster query times on these datasets. 


% \begin{table}[!t]
% \centering
% \caption{The number of class identifiers and paths.}
% %\caption{The difference between the numbers of class identifiers and paths.}
% \label{tab:numhistory}
% {\small
% \begin{tabular}{|c|r|r|r|}\hline
%       \multicolumn{1}{|c|}{Dataset}&\multicolumn{1}{|c|}{Structural} &\multicolumn{1}{|c}{IA-Structural}&\multicolumn{1}{|c|}{Path}\\ \Hline
%      {\bf Robots} & 3.3$\cdot 10^4$ & 4.3$\cdot 10^3$  & 2.5$\cdot 10^6$ \\
%      {\bf Advogato} & 2.9$\cdot 10^6$ & 1.6$\cdot 10^5$ & 8.3$\cdot 10^6$ \\
%      {\bf BioGrid} & 7.5$\cdot 10^7$  & 4.7$\cdot 10^6$  & 2.1$\cdot 10^8$ \\         
%      {\bf StringHS} & 1.7$\cdot 10^7$ & 1.0$\cdot 10^6$&  5.7$\cdot 10^8$ \\        
%      {\bf StringFC} & 9.8$\cdot 10^6$ & 3.4$\cdot 10^5$& 5.1$\cdot 10^8$\\
%      {\bf Youtube} & 2.7$\cdot 10^9$ & 6.6$\cdot 10^8$ & 3.2$\cdot 10^9$\\
%     %  {\bf YAGO} & - & 2.1$\cdot 10^6$ & - \\ 
%     %  {\bf WikiTalk} & - & 2.1$\cdot 10^6$ & - \\ 
%     %  {\bf WebGoogle} & - & 2.1$\cdot 10^6$ & - \\ 
%     %  {\bf CitPatents} & - & 2.1$\cdot 10^6$ & - \\ 
%      \hline
% \end{tabular}
% }
% \end{table}

\subsection{Are CPQ-aware indexes compact?}
\label{ssec:exp_scalability}
%We evaluate the index size and index time as scalability.
We can also give a positive answer to this question.
Table \ref{tab:index} shows the index sizes and index times.
%, and memory usages for constructing indexes.
\cpqindex{} achieves smaller index size than Path,
because it stores a single s-t pair regarding to a class while Path stores multiple s-t pairs regarding to label sequences.
\CPQ-aware indexes can reduce its size well when the graph structures and labels have large skews. 
\iacpqindex{} is much smaller than \cpqindex{} because it stores s-t pairs in the given interest.
In WikiTalk,  WebGoogle, Yago, Wikidata, and Freebase, the interest-{\it un}aware indexes cannot be constructed due to their size.
The interest-aware indexes work well for large graphs, where index size is controllable by specifying the appropriate interests. 
%IA-Structural is much smaller than IA-Path on Freebase because each path appears at multiple times in IA-Path according to the number of label sequences that each path has while at just once in IA-Structural.
%The difference between sizes of IA-Structural and IA-Path on synthetic graphs is small compared with those real graphs.

Indexing time in both \cpqindex{} and Path are generally large.
%, in particular, their memory usages are much larger than their index size. 
%It causes concerns about index construction of \cpqindex. 
%Fortunately, their index sizes are small, so it is practical that we build these indexes by using servers with rich computational resources and move them to servers for query processing.
%The index time and memory usage increase linearly as the size of graph increases, so we can . 
Comparing \cpqindex{} with Path, \cpqindex{} is less efficient than Path because \cpqindex{} requires computing $k$-path-bisimulation, while Path just enumerates s-t pairs with label sequences.
These difference is not very large in most datasets.
%Indexing time and memory usage in \cpqindex{} are generally larger than that in Path because constructing \cpqindex{} requires computing $k$-path-bisimulation, while Path just enumerates paths with label sequences.
%Thus, it is more complex than constructing Path.
Comparing the interest-aware indexes with the interest-unaware indexes, the interest-aware indexes are more practical, which clearly takes less time for construction.
\iacpqindex{} contributes to the scalable and efficient index construction with query acceleration. 
In this evaluation, we set $k$ as two. We show that \iacpqindex{} can be constructed in larger $k$ in our extended report.

%  \begin{figure*}[!t]
% \begin{minipage}{.66\textwidth}
% \vspace{-30mm}
% \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/experiment/k_query_legends.pdf}
%     \end{minipage}
%     \\
% \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=1.0\linewidth]{figures/experiment/k_query_workload_3datasets.pdf}
% \end{minipage} 
% \vspace{-7mm}
% \caption{Impact of $k$ on query time with \iacpqindex{} on YAGO, Wikidata, and Freebase}
%     \label{fig:querytime_wa_structural_index_k}
% \end{minipage}
% \begin{minipage}[t]{0.3\linewidth}
%   \centering
%   \includegraphics[width=1.0\linewidth]{figures/experiment/k_indexsize_workload.pdf}
%   \vspace{-5mm}
%   \caption{Impact of $k$ on size of \iacpqindex}
%   \label{fig:indexsize_k}   
% \end{minipage}
% \end{figure*}






% From this results, our structural index can achieve compact sizes while accelerating the conjunctive path queries. Additionally, we confirm that we can construct the interest-aware structural index for large-scale datasets.






% \subsection{Scalability}
% We here show scalability of the indexes in synthetic datasets.
% For evaluating scalability, we use synthetic datasets that have large numbers of vertices and edges.
% We cannot construct the structural index and the path index with $k=2$ even for the smallest synthetic dataset due to lacking of memory spaces.
% We here show the index size and index time of the interest-aware structural index.
% In this scalability test, we use two interest; former consists five label sequences; {\sf cites}-{\sf cites}, {\sf cites}-{\sf supervises}, {\sf publishesIn}-{\sf heldIn}, {\sf worksIn}-{\sf heldIn}$^{-1}$, and {\sf livesIn}-{\sf worksIn}$^{-1}$, and the latter consists additional five label sequences; {\sf XXXX}.

% Table \ref{tab:scalability} shows the index size and index time on each synthetic dataset.
% We confirm that we can construct the interest-aware structural index for large-scale datasets.
% The size of interest-aware index is controllable can control the size of index by specifying the appropriate index. 

%0 cites (a researcher cites a researcher)
%1 publishes in (a researcher publishes in a venue)
%2 held in (a venue is held in a city)
%3 lives in (a researcher lives in a city)
%4 works in (a researcher works in a city)
%5 supervises (a researcher supervises a researcher)

% \begin{table}[]
%     \centering
%     \caption{Scalability test}
%     \label{tab:scalability}
%     \begin{tabular}{|c|c|c|c|c|}\hline
%          \multirow{2}{*}{Dataset}& \multicolumn{2}{|c|}{workload1} & \multicolumn{2}{|c|}{workload2} \\
%           &\multicolumn{1}{c}{IS [GB]}&\multicolumn{1}{c|}{IT [sec]}&\multicolumn{1}{|c}{IS [GB]}&\multicolumn{1}{c|}{IT [sec]}\\ \Hline
%          {\bf g-Mark-1m}  & 0.4 & 79.6 & 0.8 & 166.7\\
%          {\bf g-Mark-5m}  & 2.6 & 547.4 & 5.0 & 1005.7\\
%          {\bf g-Mark-10m} & 5.6 & 1367.7 & 12.0 & 2478.0 \\
%          {\bf g-Mark-15m} & 7.8 & 5989.4  & - & - \\
%          {\bf g-Mark-20m} & 13.0 & 3380.5 & 26.0 & 7491.4 \\\hline
%     \end{tabular}
% \end{table}

% \begin{figure*}[ttt]
% \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/k_query_legends-crop.pdf}
%     \end{minipage}
%     \\
% \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/k_query_bisimulation-crop.pdf}
%     \caption{Impact of $k$ on Query time with Structural index. Note that not all indexes could be constructed within available memory.}
%     \label{fig:querytime_structural_index_k}
%     \end{minipage}
% \end{figure*}




% \begin{figure}[ttt]
%   \centering
%   \subfloat[Structural]{\epsfig{file=./figures/k_indexsize_bisimulation-crop.pdf,width=0.5\linewidth}
%   }
%     \subfloat[IA-Structural]{\epsfig{file=./figures/k_indexsize_workload-crop.pdf,width=0.5\linewidth}
%   }
%     %\subfloat[Path]{\epsfig{file=./figures/k_indexsize_path.eps,width=0.33\linewidth}
%   %\label{fig:cpu1}}

%   % \vspace{-3mm}
%   \caption{Impact of $k$ on index size}
%   \label{fig:indexsize_k}
% \end{figure}




% \begin{table*}[!t]
% \begin{minipage}[t]{.43\textwidth}
%     \centering
%     \caption{Update time on structural index}
%     \label{tab:maitenance_structural}
%     {\small
%     \begin{tabular}{|c|r|r|}\hline
%          \multirow{2}{*}{Dataset}  & \multicolumn{1}{|c|}{Edge} & \multicolumn{1}{|c|}{Edge} \\ 
%          & \multicolumn{1}{|c|}{deletion} & \multicolumn{1}{|c|}{insertion} \\\Hline
%          {\bf Robots}   & 0.0008 [s] & 0.0005 [s] \\
%          {\bf Advogato} & 0.005 [s] & 0.001 [s] \\
%          {\bf BioGrid}  & 0.6 [s] & 0.2 [s] \\         
%          {\bf StringHS} & 0.3 [s] & 0.1 [s]\\        
%          {\bf StringFC} & 0.2 [s] & 0.06 [s] \\
%          {\bf Youtube}  & 0.9 [s] & 0.3 [s]\\\hline
%     \end{tabular}
%     }
% \end{minipage}
%   %
%   \hfill
%   %
%   \begin{minipage}[t]{.565\textwidth}
%     \centering
%     \caption{Update time on IA-structural index}
%     \label{tab:maitenance_wa_structural}
%     {\small
%     \begin{tabular}{|c|r|r|r|r|}\hline
%          \multirow{2}{*}{Dataset}  & \multicolumn{1}{|c|}{Edge} & \multicolumn{1}{|c|}{Edge} & \multicolumn{1}{|c|}{Label sequence} & \multicolumn{1}{|c|}{Label sequence} \\ 
%          &\multicolumn{1}{|c|}{deletion}&\multicolumn{1}{|c|}{insertion}&\multicolumn{1}{|c|}{deletion}&\multicolumn{1}{|c|}{insertion}\\
%          \Hline
%          {\bf Robots}   & 0.0004 [s] & 0.0001 [s]& 0.2 [$\mu$s] & 0.01 [s] \\
%          {\bf Advogato} & 0.004 [s] & 0.0004 [s]& 0.3 [$\mu$s] & 0.7 [s] \\
%          {\bf BioGrid}  & 1.0 [s] & 0.005 [s]& 0.5 [$\mu$s] & 14.2 [s] \\         
%          {\bf StringHS} & 0.2 [s] & 0.03 [s]& 0.5 [$\mu$s] & 15.4 [s]\\        
%          {\bf StringFC} & 0.2 [s] & 0.04 [s]& 0.5 [$\mu$s] & 9.8 [s] \\
%          {\bf Youtube}  & 0.2 [s] & 0.1 [s]& 0.5 [$\mu$s] & 255.5 [s]\\
%          {\bf YAGO}  & 0.2 [s] & 0.04 [s]& 0.8 [$\mu$s] & 30.3 [s]\\
%          {\bf Freebase}  & 1.5 [s] & 0.2 [s]& 1.1 [$\mu$s] & 21.8 [s]\\
%          \hline
%     \end{tabular}
%     }
%     \end{minipage}
% \end{table*}





% \begin{figure*}[!t]
%   \centering
%   \begin{minipage}[t]{1.0\linewidth}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figures/experiment/k_query_legends.pdf}
%     \end{minipage}\vspace{-5mm}
% \begin{minipage}[t]{1.0\linewidth}
%   \subfloat[Query Time for structural and IA-structural on graph update and IA-structural on workload update from left, respectively]{\epsfig{file=./figures/experiment/update_query_bisimulation.pdf,width=0.6\linewidth}
%   }
%   \subfloat[Index size on graph update]{\epsfig{file=./figures/experiment/updategraph_indexsize.pdf,width=0.2\linewidth}
%   }
% \subfloat[Index size on workload update ]{\epsfig{file=./figures/experiment/interest_indexsize.pdf,width=0.2\linewidth} 
%   }
%   \caption{Impact of update on robots dataset}
%   \vspace{2mm}
%  \label{fig:maintenance}
%       \end{minipage}



\subsection{Are CPQ-aware indexes maintainable?}
\label{ssec:exp_update}
%We show that the update time and impacts of updates to performance.
In short, we can answer this question affirmatively. 
\CPQ-aware indexes can be efficiently updated with small deterioration of query processing and a small increase of its sizes.

\noindent
{\bf Update time.} 
%We update the structural index when graph is updated. In addition, we update the interest-aware structural index when we change label sequences in the interest.
%Here, we evaluate the time for index updates when edges in the graph are inserted and deleted and label sequences in the interest are inserted and deleted.
To study the impact of graph and interest updates, 
we delete and insert a hundred edges and label sequences of C2 queries, respectively, and report the average response time of each operation.
Table \ref{tab:maitenance_wa_structural} shows
the update time on \iacpqindex.
Our indexes can be quickly updated compared to the initial index construction time. 
Thus, our indexes can handle graph and interest updates on large graphs.
%Update time is highly dependent on the degrees of vertices connected to updated edges. 
%In Youtube, since the average degree is high, it takes higher time compared with the other datasets.
%The IA-Structural can be updated for graph updates more efficiently than Structural because the number of edges that are involved with graph update is smaller.
%The interest changes also can be handled with low cost.


\noindent
{\bf Impact of updates on query time and index size.}  Our update method lazily updates our index, and thus it deteriorates performance of query time and increases the index size.
We here evaluate the query time and index size after deleting $x\%$ edges (resp. $x$ label sequences) and inserting the deleted edges (resp. label sequences).
%, and after deleting $x$ label sequences in the interest and then inserting the same label sequences.

Figure \ref{fig:maintenance_querytime} shows the query time after updates.
The query templates whose query times are small (e.g., C2i and T) increase their query time after updates because of increasing {\sc LookUp} costs. 
On the other hand, the query templates with large {\sc Join} costs (e.g., C4 and Si) do not increase their query time much because lookup costs are relatively small compared with {\sc Join} costs.
Note that we confirmed that the query results are the same before and after updates.

Table \ref{tab:maintenance_indexsize} shows the increasing ratio of index size after updates.
Our update method does not merge two class identifiers even if the s-t pairs in blocks with the class identifiers are $k$-path-bisimilar, and thus the size of index increases.
We can see that our update method is practical because the increasing ratio is small even if the number of updates is large. 

% \subsection{Are CPQ-aware indexes well-behaved as $k$ grows?}
% \label{ssec:exp_analysis}
% We can also give a positive answer.
% Figure~\ref{fig:querytime_wa_structural_index_k} shows the query time for \iacpqindex{} varying with $k$.
% We can see that the query time decreases from $k=1$ to $k=2$. Some query times increase when $k>2$. There are two reasons for this. First, CPQ-aware indexes divide paths into too fine granularity for some query templates, and which increases {\sc LookUp} and {\sc Conjunction} costs.
% Second, costs of {\sc Join} possibly increase, in particular, query time of C4 and Si queries increases when $k=3$. 
% As we described in Section~\ref{ssec:indexdef}, queries with diameters $i$ become the fastest when $k = i$. 
% %We here note that query time of $k=1$ is equivalent to query time that queries are outside of interests.

% Figure \ref{fig:indexsize_k} shows the index size of \iacpqindex{} varying with $k$.
% The index size increases with increasing $k$ generally.
% The increase ratio depends on the number of paths stored in \iacpqindex.
% Therefore, the size of \iacpqindex{} often slightly increases from $k=3$ to $k=4$ because the numbers of length 3 paths and length 4 paths are similar.
% In particular, the index size in Freebase does not increase much even when $k$ increases.
% We do not show the result of the index time in detail; the index time increases as $k$ grows.

% For deciding appropriate $k$, we can generally select the maximum length of interests when building \iacpqindex.
% Otherwise, we select $k$ and the interests to control index construction costs.

==> algorithms/maintance_edgedelete.tex <==
\begin{algorithm}[!t] 
	\caption{Update for edge deletion}	\label{alg:deleteedge}
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	            \SetKwFunction{Expand}{Expand}
	            \Input{Index $I_{[\graph]_k}$, \graph, deleted edge $e_d = (v,u,\elabel)$}
	            \Output{Updated Index}
            	{\bf procedure} {\sc EdgeDeletion}\\
            	$\spaths \leftarrow$ Enumerate paths at most length $k$ involving $e_d$;\\
            	\For{$(x,y) \in \spaths$}{
                	\If{there are alternative paths of $(x,y)$}{
                	    Remove $(x,y)$ from $\spaths$;
                	}
            	}
            	\For{$(x,y) \in \spaths$}{
                	insertflag$\leftarrow$ false;\\
                	\For{$h \in \histories$}{
                	    \If{$(x,y) \in I_{h2p}(h)$}{
                	    delete $(x,y)$ from $I_{h2p}(h)$;\\
                	    $h_d \leftarrow h$;\\
                	    {\bf break};\\
                	    }
                	}
                 	\For{$\overline{\elabel} \in \elabels^{\leq k}$}{
                     	\For{$h \in I_{l2h}(\overline{\elabel})$}{
                     	    \If{$h = h_d$ and $\overline{\elabel} \not\in \elabels^{\leq k}(x,y)$}{
                     	        $h_{new}\leftarrow$ new history identifier;\\ 
                     	        $I_{l2h}$.append($\overline{\elabel}, h_{new}$);\\
                     	        insertflag$\leftarrow$ true;\\
                     	    }
                 	    }
                 	}
                 	\If{insertflag}{
                 	    $I_{h2p}$.append($h_{new},(x,y)$);}
             	}
              {\bf return} $I_{[\graph]_k}$;\\
              {\bf end procedure}
\end{algorithm}


==> algorithms/query.tex <==
\begin{algorithm}[!t] 
	\caption{Query processing}	\label{alg:querywhole}
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	            \Input{Node on query tree $q$, \cpqindex $I$}
	            \Output{set of paths $\spaths$, set of histories $\shistories$}
            	{\bf procedure}  {\sc Evaluation}($q$, $I$)\\	
        	    \If{operation is  {\sc LookUp}}{
        	        {\bf return} {\sc LookUp ($q.\overline{\elabel}$, $I$);}
        	    }
        	    \ElseIf{operation is {\sc Identify}}{
            	    {\bf return} {\sc Identify}($\spaths, \shistories$, $I$);
        	    }
            	\Else{
            	    $\spaths _l , \shistories _l \leftarrow$ {\sc Evaluation}($q_l$, $I$);\\
                    $\spaths _r, \shistories_r \leftarrow$ {\sc Evaluation}($q_r$, $I$);\\
                    \If{operation of $q$ is {\sc Join}}{
                	    {\bf return} {\sc Join} ($\spaths _l, \spaths _r, \shistories_l, \shistories_r$, $I$);
                	}
            	    \ElseIf{operation of $q$ is {\sc Conjunction}}{
            	        {\bf return} {\sc Conjunction} ($\spaths _l, \spaths _r, \shistories_l, \shistories_r$, $I$);
            	    }
              }
              \If{$q$ is the root of query tree}{
                $\spaths \leftarrow \spaths \cup I_{h2p}(h)$ for all $h \in \shistories$;
              }
              {\bf return} $\spaths, \shistories$;\\
              {\bf end procedure}
\end{algorithm}

\begin{algorithm}[!t] 
	\caption{Operations}	\label{alg:queryoperation}
		\DontPrintSemicolon
              {\bf procedure} {\sc LookUp($\overline{\elabel}$, $I$)}\\
            %   \If{length of \elabel is larger than $k$}{
            % 	  divide the label sequences into $\elabel_1$ and $\elabel_2$;\\
            % 	  $n_1 \leftarrow access (\elabel_1)$;
            % 	  $n_2 \leftarrow access (\elabel_2)$;\\
            % 	  {\bf return} {\sc Join}({\sc Evaluation}($n_1$, $I$),{\sc Evaluation}($n_2$, $I$));\\
            %   }
              {\bf return} $\emptyset, I_{l2p}(\overline{\elabel})$;\\
              \hrulefill \\
              {\bf procedure} {\sc Join}($\spaths _l, \spaths _r, \shistories _l, \shistories _r$, $I$)\\
              $\spaths_l \leftarrow \{(v_s,v_t) \mid (v_s,v_t) \in I_{h2p}(h) \land h \in \shistories _l \}$;\\
              $\spaths_r \leftarrow \{(v_s,v_t) \mid (v_s,v_t) \in I_{h2p}(h) \land h \in \shistories _r \}$;\\
              sort $\spaths_l$ in ascending order of target of paths;\\
              sort $\spaths_r$ in ascending order of sources of paths;\\
              $\spaths \leftarrow \{(v_s,v_t')\mid (v_s,v_t) \in \spaths _l \land (v_s',v_t') \in \spaths _r \land v_t=v_s' \}$\\
              {\bf return} $\spaths, \emptyset$;\\
              \hrulefill \\
              {\bf procedure} {\sc Conjunction}($\spaths _l, \spaths _r, \shistories _l, \shistories _r$, $I$)\\
              \If{$\shistories _l \neq \emptyset$ and $\shistories _r \neq \emptyset$}{
                $\shistories \leftarrow \shistories_l \cap \shistories_r$;\\
                {\bf return} $\emptyset, \shistories$;\\
              }
              \Else{
                \If{$\spaths _l \neq \emptyset$} {
                    $\spaths _l \leftarrow \{(v_s,v_t) \mid (v_s,v_t) \in I_{h2p}(h) \land h \in \shistories _l \}$;\\
                    sort $\spaths _l$ in ascending order of target of paths;\\
                }
                \If{$\spaths _r \neq \emptyset$}{ 
                    $\spaths _r \leftarrow \{(v_s,v_t) \mid (v_s,v_t) \in I_{h2p}(h) \land h \in \shistories _r \}$;\\
                    sort $\spaths _r$ in ascending order of sources of paths;\\
                }
                $\spaths \leftarrow \spaths _l \cap \spaths _r$;\\
                {\bf return} $\spaths, \emptyset$;
              }
              \hrulefill \\
              {\bf procedure} {\sc Identify}($\spaths,  \shistories$, $I$)\\
                \If{$\shistories \neq \emptyset$}{
                    $\shistories' \leftarrow \{h \mid h \in \shistories \land (v_s,v_t) \in I_{h2p}(h) \land v_s=v_t\}$;\\
                    {\bf return} $\emptyset, \shistories'$;
                }
                \Else{
                    $\spaths' \leftarrow \{(v_s,v_t) \mid (v_s,v_t) \in \spaths \land v_s=v_t\}$;\\
                    {\bf return} $\spaths', \emptyset$;
                    }
\end{algorithm}


==> bisimulation_tikz.tex <==

\begin{figure*}[ttt]
    \centering
    \scalebox{0.6}{
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,
  thick,main node/.style={circle,draw,font=\sffamily\small}]

        scale only axis,
        width             = 6.5cm,
        enlarge y limits  = {abs=0.5},
        axis y line*      = middle,
        y axis line style = dashed,
        ytick             = \empty,
        axis x line*      = bottom
      ]
  %\draw[step=0.5,very thin, gray] (-1,-2) grid (28,4.5);
  %thick,main node/.style={circle,fill=blue!20,draw,font=\sffamily\large}]

  %\node[above right] at (0,15.25)  {\large 1-path-bisumulation};
    \node at (10,3.6) {\Large $\paths^{\leq1}$};
    \node at (10,3.3)  {\Large  $\overbrace{\qquad \qquad\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad}^{}$};
    
    \node at (24,3.6) {\Large $\paths^{\leq2} - \paths^{\leq1}$};
    \node at (24,3.3)  {\Large  $\overbrace{\qquad \qquad \qquad\qquad \qquad \qquad \qquad \qquad}^{}$};
%   1-path-bisumulation
  \coordinate (1) at (0,1.5);
  \draw ($(1)+(0,0)$) rectangle ($(1)+(28,1.5)$);
  \foreach \point in {2,8,12,16,18,20} {\draw[-] ($(1)+(\point,0)$) -- ($(1)+(\point,1.5)$);}
   \node at ($(1)+(-0.5,0.75)$)  {\large k=1};
  \node at ($(1)+(1,0.75)$)  {\large (ada,ada)};
  \node at ($(1)+(3,1)$)  {\large (tim,tim)};
  \node at ($(1)+(3,0.5)$)  {\large (zoe,zoe)};
  \node at ($(1)+(5,1)$)  {\large (sue,sue)};
  \node at ($(1)+(5,0.5)$)  {\large (liz,liz)}; 
  \node at ($(1)+(7,0.75)$)  {\large (joe,joe)};
  \node at ($(1)+(9,0.75)$)  {\large (ada,tim)};
  \node at ($(1)+(11,0.75)$)  {\large (joe,zue)};     
  \node at ($(1)+(13,0.75)$)  {\large (tim,ada)};
  \node at ($(1)+(15,0.75)$)  {\large (zoe,joe)};  
  \node at ($(1)+(17,1)$)  {\large (tim,sue)};
  \node at ($(1)+(17,0.5)$)  {\large (zoe,liz)};  
  \node at ($(1)+(19,1)$)  {\large (sue,tim)};
  \node at ($(1)+(19,0.5)$)  {\large (liz,zoe)};  
  \node at ($(1)+(21,1)$)  {\large (ada,sue)};
  \node at ($(1)+(21,0.5)$)  {\large (joe,liz)};  
  \node at ($(1)+(23,1)$)  {\large (sue,ada)};
  \node at ($(1)+(23,0.5)$)  {\large (liz,joe)};  
  \node at ($(1)+(25,1)$)  {\large (tim,liz)};
  \node at ($(1)+(25,0.5)$)  {\large (zoe,sue)};  
  \node at ($(1)+(27,1)$)  {\large (liz,tim)};
  \node at ($(1)+(27,0.5)$)  {\large (sue,zoe)};  

%   2-path-bisumulation
  \draw (0,0) rectangle (28,1.5);
  \foreach \point in {2, 4, 6,8,10,12,14,16,18,20,22,24,26} {\draw[-] (\point,0) -- (\point,1.5);}
  \node at (-0.5,0.75)  {\large k=2};
  
  \node at (1,0.75)  {\large (ada,ada)};
  \node at (3,1)  {\large (tim,tim)};
  \node at (3,0.5)  {\large (zoe,zoe)};
  \node at (5,1)  {\large (sue,sue)};
  \node at (5,0.5)  {\large (liz,liz)}; 
  \node at (7,0.75)  {\large (joe,joe)};
  \node at (9,0.75)  {\large (ada,tim)};
  \node at (11,0.75)  {\large (joe,zue)};     
  \node at (13,0.75)  {\large (tim,ada)};
  \node at (15,0.75)  {\large (zoe,joe)};  
  \node at (17,1)  {\large (tim,sue)};
  \node at (17,0.5)  {\large (zoe,liz)};  
  \node at (19,1)  {\large (sue,tim)};
  \node at (19,0.5)  {\large (liz,zoe)};  
  \node at (21,1)  {\large (ada,sue)};
  \node at (21,0.5)  {\large (joe,liz)};  
  \node at (23,1)  {\large (sue,ada)};
  \node at (23,0.5)  {\large (liz,joe)};  
  \node at (25,1)  {\large (tim,liz)};
  \node at (25,0.5)  {\large (zoe,sue)};  
  \node at (27,1)  {\large (liz,tim)};
  \node at (27,0.5)  {\large (sue,zoe)};  
  
%   example of paths  
  \node at (2.5,-0.5)  {\large Examples of paths of length two};
  \node[text width=1.75cm,text centered]at (1,-1.25){ (tim,tim)\\(zoe, zoe)};
  \draw[dashed] (0,-0.75) rectangle (8,-2.75);
  \node[main node] (110)  at (4.5,-1.25) {tim};
  \node[main node] (111)  [left of=110] {ada};
  \node[main node] (112)  at (5.5,-1.25) {tim};
  \node[main node] (113)  [right of=112] {sue};
  \node[main node] (114)  at (4.5,-2.25) {zoe};
  \node[main node] (115)  [left of=114] {joe};
  \node[main node] (116)  at (5.5,-2.25) {zoe};
  \node[main node] (117)  [right of=116] {liz};
  
  \node[text width=1.75cm,text centered]at (9.5,-1.25){ (joe,joe)};
  \draw[dashed] (8.5,-0.75) rectangle (13.5,-2.75);
  \node[main node] (160)  at (13,-1.75) {zoe};
  \node[main node] (161)  [left of=160] {joe};
  
  \node[text width=1.75cm,text centered]at (15,-1.25){ (tim,ada)};
  \draw[dashed] (14,-0.75) rectangle (19.5,-2.75);
  \node[main node] (100)  at (19,-1.75) {tim};
  \node[main node] (101)  [left of=100] {ada};

  %\draw[dashed] (20,-0.5) rectangle (22,-2.5);

  \node[text width=1.75cm,text centered]at (21,-1.25){ (ada,sue)\\(joe, liz)};
  \draw[dashed] (20,-0.75) rectangle (27,-2.75);
  \node[main node] (90)  at (24.5,-1.25) {tim};
  \node[main node] (91)  [left of=90] {ada};
  \node[main node] (92)  at (24.5,-2.25) {zoe};
  \node[main node] (93)  [left of=92] {joe};
  \node[main node] (94)  [right of=90] {sue};
  \node[main node] (95)  [right of=92] {liz};
  

  \path[every node/.style={font=\small}]
    %   (10) edge [loop left]  node[above] {} (10)
       
    %   (20) edge [bend right] node[left] {} (21)
    %   (21) edge [bend right] node[left] {} (20)
    %   (22) edge [bend right] node[left] {} (23)
    %   (23) edge [bend right] node[left] {} (22)
       
    %   (30) edge [bend right] node[left] {} (31)
    %   (31) edge [bend right] node[left] {} (30)
    %   (32) edge [bend right] node[left] {} (33)
    %   (33) edge [bend right] node[left] {} (32)
       

    %   (41) edge [left] node[left] {} (40)
    %   (43) edge [left] node[left] {} (42)
       
    %   (51) edge [left] node[left] {} (50)
    %   (53) edge [left] node[left] {} (52)
       
    %   (63) edge [bend right] node[left] {} (61)
    %   (62) edge [bend right] node[left] {} (60)
    %   (60) edge [bend right] node[left] {} (62)
    %   (61) edge [bend right] node[left] {} (63)
       
    %   %   2-path-bisumulation
       
    %   (71) edge [bend right] node[left] {} (72)
    %   (72) edge [bend right] node[left] {} (71)
    %   (70) edge [loop left]  node[above] {} (70)
       
    %   (81) edge [bend right] node[left] {} (80)
    %   (80) edge [bend right] node[left] {} (81)
    %   (81) edge [loop left]  node[above] {} (81)
       
       (91) edge [bend right] node[above] {\edgefont{r}} (90)
       (90) edge [bend right] node[below] {\edgefont{w}} (91)
       (92) edge [bend right] node[below] {\edgefont{w}} (93)
       (93) edge [bend right] node[above] {\edgefont{r}} (92)
       (90) edge [left] node[below] {\edgefont{w}} (94)
       (92) edge [left] node[below] {\edgefont{w}} (95)
       
      (101) edge [bend right] node[above] {\edgefont{r}} (100)
      (100) edge [bend right] node[below] {\edgefont{w}} (101)
      (101) edge [loop left]  node[below] {\edgefont{r}} (101)
       
      (111) edge [bend right] node[above] {\edgefont{r}} (110)
      (110) edge [bend right] node[below] {\edgefont{w}} (111)
      (112) edge [left] node[below] {\edgefont{w}} (113)
      (115) edge [bend right] node[above] {\edgefont{r}} (114)
      (114) edge [bend right] node[below] {\edgefont{w}} (115)
      (116) edge [left] node[below] {\edgefont{w}} (117)
       
    %   (121) edge [left] node[left] {} (120)
    %   (122) edge [bend right] node[left] {} (120)
    %   (120) edge [bend right] node[left] {} (122)
    %   (124) edge [left] node[left] {} (123)
    %   (123) edge [bend right] node[left] {} (125)
    %   (125) edge [bend right] node[left] {} (123)
       
    %   (131) edge [bend right] node[left] {} (130)
    %   (130) edge [bend right] node[left] {} (131)
    %   (132) edge [bend right] node[left] {} (133)
    %   (133) edge [bend right] node[left] {} (132)
    %   (130) edge [left] node[left] {} (134)
    %   (132) edge [left] node[left] {} (135)
       
    %   (143) edge [bend right] node[left] {} (141)
    %   (142) edge [bend right] node[left] {} (140)
    %   (140) edge [bend right] node[left] {} (142)
    %   (141) edge [bend right] node[left] {} (143)
       
    %   (151) edge [left] node[left] {} (150)
    %   (152) edge [bend right] node[left] {} (150)
    %   (150) edge [bend right] node[left] {} (152)
    %   (154) edge [left] node[left] {} (153)
    %   (153) edge [bend right] node[left] {} (155)
    %   (155) edge [bend right] node[left] {} (153)
       
       (161) edge [bend right] node[above] {\edgefont{r}} (160)
       (160) edge [bend right] node[below] {\edgefont{w}} (161);

%   \node[draw,text width=1.75cm,text centered,very thick]at (1.5,12.5){ada $\to$ tim\\joe $\to$ zoe};
%   \draw[dashed] (3,11.5) rectangle (6,13.5);
%   \node[main node] (20)  at (5.5,13) {tim};
%   \node[main node] (21)  [left of=20] {ada};
%   \node[main node] (22)  at (5.5,12) {zoe};
%   \node[main node] (23)  [left of=22] {joe};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (1.5,10.25){ tim $\to$ ada\\zoe $\to$ joe};
%   \draw[dashed] (3,9) rectangle (6,11);
%   \node[main node] (30)  at (5.5,10.5) {tim};
%   \node[main node] (31)  [left of=30] {ada};
%   \node[main node] (32)  at (5.5,9.5) {zoe};
%   \node[main node] (33)  [left of=32] {joe};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (1.5,7.5){tim $\to$ sue\\zoe $\to$ liz};
%   \draw[dashed] (3,6.5) rectangle (6,8.5);
%   \node[main node] (40)  at (5.5,8) {sue};
%   \node[main node] (41)  [left of=40] {tim};
%   \node[main node] (42)  at (5.5,7) {liz};
%   \node[main node] (43)  [left of=42] {zoe};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (1.5,5){ sue $\to$ tim\\liz $\to$ zoe};
%   \draw[dashed] (3,4) rectangle (6,6);
%   \node[main node] (50)  at (5.5,5.5) {sue};
%   \node[main node] (51)  [left of=50] {tim};
%   \node[main node] (52)  at (5.5,4.5) {liz};
%   \node[main node] (53)  [left of=52] {zoe};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (1.5,2){ liz $\to$ sue\\sue $\to$ liz};
%   \draw[dashed] (3,0.5) rectangle (6,3.5);
%   \node[main node] (60)  at (5.5,3) {sue};
%   \node[main node] (61)  [left of=60] {sue};
%   \node[main node] (62)  [below of=60] {liz};
%   \node[main node] (63)  [below of=61] {liz};

% %   2-path-bisumulation
%   \draw (6.9,0) rectangle (28,16);
%   \node[above right] at (6.9,15.25)  {\large 2-path-bisumulation};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (8.5,14.5){ada $\to$ ada};
%   \draw[dashed] (10,14) rectangle (16,15);
%   \node[main node] (70)  at (12,14.5) {ada};
%   \node[main node] (71)  at (13.25,14.5) {ada};
%   \node[main node] (72)  [right of=71] {tim};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (8.5,12.75){ada $\to$ tim};
%   \draw[dashed] (10,12.25) rectangle (16,13.25);
%   \node[main node] (80)  at (14,12.75) {tim};
%   \node[main node] (81)  [left of=80] {ada};

%   \node[draw,text width=1.75cm,text centered,very thick]at (8.5,10.5){ada $\to$ sue\\joe $\to$ liz};
%   \draw[dashed] (10,9.5) rectangle (16,11.5);
%   \node[main node] (90)  at (13,11) {tim};
%   \node[main node] (91)  [left of=90] {ada};
%   \node[main node] (92)  at (13,10) {zoe};
%   \node[main node] (93)  [left of=92] {joe};
%   \node[main node] (94)  [right of=90] {sue};
%   \node[main node] (95)  [right of=92] {liz};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (8.5,8.25){ tim $\to$ ada};
%   \draw[dashed] (10,7.75) rectangle (16,8.75);
%   \node[main node] (100)  at (14,8.25) {tim};
%   \node[main node] (101)  [left of=100] {ada};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (8.5,6){ tim $\to$ tim\\zoe $\to$ zoe};
%   \draw[dashed] (10,5) rectangle (16,7);
%   \node[main node] (110)  at (12.5,5.5) {zoe};
%   \node[main node] (111)  [left of=110] {joe};
%   \node[main node] (112)  at (13.5,5.5) {zoe};
%   \node[main node] (113)  [right of=112] {liz};
%   \node[main node] (114)  at (12.5,6.5) {tim};
%   \node[main node] (115)  [left of=114] {ada};
%   \node[main node] (116)  at (13.5,6.5) {tim};
%   \node[main node] (117)  [right of=116] {sue};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (8.5,2.75){ tim $\to$ liz\\zoe $\to$ sue};
%   \draw[dashed] (10,1.25) rectangle (16,4.25);
%   \node[main node] (120)  at (12.5,3.75) {sue};
%   \node[main node] (121)  [left of=120] {tim};
%   \node[main node] (122)  [below of=120] {liz};
%   \node[main node] (123)  at (15.5,1.75) {liz};
%   \node[main node] (124)  [left of=123] {zoe};
%   \node[main node] (125)  [above of=123] {sue};

% %   2-path-bisumulation right
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (18.75,14){ sue $\to$ ada\\liz $\to$ joe};
%   \draw[dashed] (20.25,13) rectangle (26.25,15);
%   \node[main node] (130)  at (23.25,13.5) {tim};
%   \node[main node] (131)  [left of=130] {ada};
%   \node[main node] (132)  at (23.25,14.5) {zoe};
%   \node[main node] (133)  [left of=132] {joe};
%   \node[main node] (134)  [right of=130] {sue};
%   \node[main node] (135)  [right of=132] {liz};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (18.75,10.75){ sue $\to$ sue\\liz $\to$ liz};
%   \draw[dashed] (20.25,9.25) rectangle (26.25,12.25);
%   \node[main node] (140)  at (24.25,11.75) {sue};
%   \node[main node] (141)  [left of=140] {sue};
%   \node[main node] (142)  [below of=140] {liz};
%   \node[main node] (143)  [below of=141] {liz};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (18.75,7){ sue $\to$ zoe\\liz $\to$ tim};
%   \draw[dashed] (20.25,5.5) rectangle (26.25,8.5);
%   \node[main node] (150)  at (22.75,8) {sue};
%   \node[main node] (151)  [left of=150] {tim};
%   \node[main node] (152)  [below of=150] {liz};
%   \node[main node] (153)  at (25.75,6) {liz};
%   \node[main node] (154)  [left of=153] {zoe};
%   \node[main node] (155)  [above of=153] {joe};
  
%   \node[draw,text width=1.75cm,text centered,very thick]at (18.75,4.25){ joe $\to$ joe};
%   \draw[dashed] (20.25,3.75) rectangle (26.25,4.75);
%   \node[main node] (160)  at (24.25,4.25) {zoe};
%   \node[main node] (161)  [left of=160] {joe};
  
%   \path[every node/.style={font=\small}]
%       (10) edge [loop left]  node[above] {} (10)
       
%       (20) edge [bend right] node[left] {} (21)
%       (21) edge [bend right] node[left] {} (20)
%       (22) edge [bend right] node[left] {} (23)
%       (23) edge [bend right] node[left] {} (22)
       
%       (30) edge [bend right] node[left] {} (31)
%       (31) edge [bend right] node[left] {} (30)
%       (32) edge [bend right] node[left] {} (33)
%       (33) edge [bend right] node[left] {} (32)
       

%       (41) edge [left] node[left] {} (40)
%       (43) edge [left] node[left] {} (42)
       
%       (51) edge [left] node[left] {} (50)
%       (53) edge [left] node[left] {} (52)
       
%       (63) edge [bend right] node[left] {} (61)
%       (62) edge [bend right] node[left] {} (60)
%       (60) edge [bend right] node[left] {} (62)
%       (61) edge [bend right] node[left] {} (63)
       
%       %   2-path-bisumulation
       
%       (71) edge [bend right] node[left] {} (72)
%       (72) edge [bend right] node[left] {} (71)
%       (70) edge [loop left]  node[above] {} (70)
       
%       (81) edge [bend right] node[left] {} (80)
%       (80) edge [bend right] node[left] {} (81)
%       (81) edge [loop left]  node[above] {} (81)
       
%       (91) edge [bend right] node[left] {} (90)
%       (90) edge [bend right] node[left] {} (91)
%       (92) edge [bend right] node[left] {} (93)
%       (93) edge [bend right] node[left] {} (92)
%       (90) edge [left] node[left] {} (94)
%       (92) edge [left] node[left] {} (95)
       
%       (101) edge [bend right] node[left] {} (100)
%       (100) edge [bend right] node[left] {} (101)
%       (101) edge [loop left]  node[above] {} (101)
       
%       (111) edge [bend right] node[left] {} (110)
%       (110) edge [bend right] node[left] {} (111)
%       (112) edge [left] node[left] {} (113)
%       (115) edge [bend right] node[left] {} (114)
%       (114) edge [bend right] node[left] {} (115)
%       (116) edge [left] node[left] {} (117)
       
%       (121) edge [left] node[left] {} (120)
%       (122) edge [bend right] node[left] {} (120)
%       (120) edge [bend right] node[left] {} (122)
%       (124) edge [left] node[left] {} (123)
%       (123) edge [bend right] node[left] {} (125)
%       (125) edge [bend right] node[left] {} (123)
       
%       (131) edge [bend right] node[left] {} (130)
%       (130) edge [bend right] node[left] {} (131)
%       (132) edge [bend right] node[left] {} (133)
%       (133) edge [bend right] node[left] {} (132)
%       (130) edge [left] node[left] {} (134)
%       (132) edge [left] node[left] {} (135)
       
%       (143) edge [bend right] node[left] {} (141)
%       (142) edge [bend right] node[left] {} (140)
%       (140) edge [bend right] node[left] {} (142)
%       (141) edge [bend right] node[left] {} (143)
       
%       (151) edge [left] node[left] {} (150)
%       (152) edge [bend right] node[left] {} (150)
%       (150) edge [bend right] node[left] {} (152)
%       (154) edge [left] node[left] {} (153)
%       (153) edge [bend right] node[left] {} (155)
%       (155) edge [bend right] node[left] {} (153)
       
%       (161) edge [bend right] node[left] {} (160)
%       (160) edge [bend right] node[left] {} (161);
\end{tikzpicture}
}
    \caption{1-path-bisimuation and 2-path-bisimulation equivalence of paths in $\graph_{ex}$ of Figure \ref{fig:graph}}
    \label{fig:bisimulation_example}
\end{figure*}



==> intro_bigpicture_tikz.tex <==


\begin{figure}[ttt]
    \centering
    \scalebox{0.6}{
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,
  thick,main node/.style={draw,rectangle,rounded corners=3pt, minimum height = 1.5cm,  minimum width = 6cm, rotate=90}]

        scale only axis,
        width             = 6.5cm,
        enlarge y limits  = {abs=0.5},
        axis y line*      = middle,
        y axis line style = dashed,
        ytick             = \empty,
        axis x line*      = bottom
      ]
     
  %\draw[step=0.5,very thin, gray] (0,0) grid (30,15);
  %thick,main node/.style={circle,fill=blue!20,draw,font=\sffamily\large}]
  %\draw (0,0) rectangle (10,2);
  %\node[above right] at (1,1)  {Q in Sparck, ...};

%   1-path-bisumulation
  \node[main node] (1)  at (0,0) {\LARGE Query $Q$ $\in$ SPARQL, Cypher, ...};
  \node[main node ,align=left] (2)  at (3,0) {\LARGE \cpq{} subqueries $Q_1$, $Q_2,$ $\ldots,$ $Q_n$ \\ \LARGE with execution plans};
  \node[main node] (3)  at (6,0) {\LARGE Query evaluation with index};
  \node[main node] (4)  at (9,0) {\LARGE Results of $Q$};
  \node[ rotate=90] at (1.5,0.8) {\LARGE Compile $Q$};
    \node[ rotate=90] at (4.5,0.8) {\LARGE Process};
      \node[ rotate=90] at (7.5,0.8) {\LARGE Combine};
   \path[every node/.style={font=\LARGE}]
   (1) edge [left] node[left] {} (2)
   (2) edge [left] node[left] {} (3)
   (3) edge [left] node[left] {} (4);
\end{tikzpicture}
}
    \caption{Query processing flow}
    \label{fig:bisimulation_example_appendix}
\end{figure}


